Hogwild! over Distributed Local Data Sets with Linearly Increasing Mini-Batch Sizes

Hogwild! implements asynchronous Stochastic Gradient Descent (SGD) where multiple threads in parallel access a common repository containing training data, perform SGD iterations and update shared state that represents a jointly learned (global) model. We consider big data analysis where training data is distributed among local data sets in a heterogeneous way -- and we wish to move SGD computations to local compute nodes where local data resides. The results of these local SGD computations are aggregated by a central "aggregator" which mimics Hogwild!. We show how local compute nodes can start choosing small mini-batch sizes which increase to larger ones in order to reduce communication cost (round interaction with the aggregator). We improve state-of-the-art literature and show $O(\sqrt{K}$) communication rounds for heterogeneous data for strongly convex problems, where $K$ is the total number of gradient computations across all local compute nodes. For our scheme, we prove a \textit{tight} and novel non-trivial convergence analysis for strongly convex problems for {\em heterogeneous} data which does not use the bounded gradient assumption as seen in many existing publications. The tightness is a consequence of our proofs for lower and upper bounds of the convergence rate, which show a constant factor difference. We show experimental results for plain convex and non-convex problems for biased (i.e., heterogeneous) and unbiased local data sets.

==> Section/02_Relatedwork.tex <==
\section{Related Work}

We assume there are $K$ clients over which the data is partitioned, with $\mathscr{D}_{k}$ \footnote{In FL setting, the data distribution could be IID or non-IID and may have unbalanced property.} is the set of indexes of data points on client $k$ and the number of available samples on client $k$ is $n_k = \lvert{\ \mathscr{D}_k}\rvert$. A federated learning system is a learning process where the total $K$ clients collaboratively train a global model $w$ and client $k$ does not exchange its own local data $\mathscr{D}_k$ to other clients or server. In particular, the goal is typically to minimize the following objective function \cite{mcmahan,chen2019fedhealth}:
\begin{equation}
    \min_{w \in \mathbb{R}^{d}}{F(w)} = \sum_{k=1}^{K} \frac{n_k}{n} F_k(w)\label{eq6}
\end{equation}
with $F_{k}$ is the local loss function in client $k$, specifically:
\begin{equation}
F_{k}(w) = \frac{1}{n_k} \sum_{i \in \mathscr{D}_k} f_i(w)
\end{equation}
From the perspective of accuracy \cite{yang2019federated}, we define $\mathscr{D} = \mathscr{D}_1 \cup \mathscr{D}_2 ... \cup \mathscr{D}_K$ and the accuracy of model over $\mathscr{D}$ is $\mathscr{A}_\mathscr{D}$ and the accuracy of model using FL is $\mathscr{A}_{fl}$. Formally, we say the federated learning has $\epsilon$-accuracy if the following requirement is satisfied: $\lvert{\ \mathscr{A}_\mathscr{D} - \mathscr{A}_{fl} }\rvert < \epsilon$.




==> Section/04_Convergence_Analysis.tex <==
\section{Convergence Analysis}

\subsection{Convergence Analysis of Hogwild!}


==> Section/05_Experiment.tex <==
\section{Experiment}
\label{sec:experiment}

Without loss of generality, we implement SGD and Hogwild! algorithms with constant step sizes. Moreover, it is sufficient to only consider our $k$-round asynchronous FL where the clients run SGD with constant step sizes because this is the most practical setup. We use Python and Tensorflow in our programming. 

\textcolor{red}{Ha to Nhuong: need to describe everything in detail. For example, how many samples in the training datasets. What is the configuration of clients and system. How do you implement Hogwild!, i.e., how to implement the memory lock for atomic reads and writes. What is the delay we introduce for atomic reads/ writes in the simulation.}

In this paper, we mainly focus on convex problem in machine learning, especially logistic regression problem with $\ell_{2}$ regularization.

The weight $w$ of the logistic function can be learned by minimizing the log-likelihood function $J$ (the logistic regression loss function) through gradient descent.
\begin{equation} \label{eq_logstic_reg}
    J = - \sum_{i}^N [ y_{i} \cdot \log (\sigma_i) + (1 - y_{i}) \cdot \log (1 - \sigma_i) ] + \frac{\lambda}{2}\norm{w}^{2},
\end{equation}
where $N$ is the number of training samples, $\lambda$ is regularization parameter, $\sigma$ is a sigmoid function with parameters weight $w$, bias value $b$ and input data $x$ defined as:
\begin{equation} \label{eq_sigmoid}
    \sigma(w, x, b) = \frac{1}{1 + e^{-(w^{\mathrm{T}}x + b)}}.
\end{equation}

\subsection{Simulation of SGD and Hogwild! and their comparison}
\label{subsec:hogwild_simu}

We consider the binary classification for digits $0$ and $1$ for MNIST dataset. The goal of this experiment is to study the behavior of Hogwild! and the limitation of delay variable $\tau$. \textcolor{red}{For simulating the atomic read and write operation, we partition the full model $w$ into $m$ parts and these parts are locked by synchronized lock to guarantee the atomic operation. Moreover, in order to simulate the delay of read and write operation, we define atomic read and write operation will take 2 milliseconds, 1 millisecond respectively.} The detail sett up of the experiments is described below:
\begin{table}[ht]
\caption{Hogwild! training parameters}
\label{tbl_hogwild}
\vskip 0.1in
\begin{center}
\begin{small}
% \begin{sc}
\begin{tabular}{lcccr}
\toprule
Parameter & Value & Notes \\ [0.5ex]
\midrule

Regularization parameter $\lambda$   & 1/$N$ &    \\
Learning rate $\eta$ & 0.001 &  fixed                       \\ 
% \hline
Data set & MNIST & $0$ and $1$ digit                \\
%Size of Dataset & ????&   \\

% \hline
Number of atomic writes & 50000 &                       \\
% \hline
Image size & 28x28   & grayscale                        \\
Data set records $N$ & 14867 &                          \\
% \hline
Number of threads $n$ & 1/3/5/10/15/20 &                  \\
% \hline
Number of masks $m$ & 14 &                               \\
% \hline
Epoch & 20 &                                            \\
\bottomrule
\end{tabular}
% \end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

\begin{figure}[hbt]
  \centering
  \begin{minipage}[b]{0.5\textwidth}
 \includegraphics[width=\columnwidth,keepaspectratio]{tikz/04_hogwild_and_sgd_train_loss.PNG}
\caption{The training loss at the end of each epoch.}
\label{fig:hogwild_train_err}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.5\textwidth}
 \includegraphics[width=\columnwidth,keepaspectratio]{tikz/03_hogwild_and_sgd_train_duration.PNG}
\caption{Average training duration with different number of threads.}
\label{fig:hogwild_duation}
  \end{minipage}
\end{figure}

Figures~\ref{fig:hogwild_train_err} and \ref{fig:hogwild_duation} show the training error and speedup rate for training process using the Hogwild! algorithm. When n$\_$thread=1, Hogwild! is exactly SGD. As can be seen from Figure~\ref{fig:hogwild_train_err}, while the number of threads increases, the values of training error for all threads are nearly the same. It means that single thread SGD and Hogwild! with multiple threads have the same accuracy or training error. In contrast to Figure~\ref{fig:hogwild_train_err}, we see a significant decrease of training duration when the number of threads goes up. However, the number of joined threads needs to be reasonable due to the limit of max delay $\tau$ and the number of masks, which can reduce the performance of training process due to the effect of collision in atomic read and atomic write constraints. For example, when n$\_$thread=20, the duration increases instead of decreasing due to the effect of atomic read or write. 

\subsection{Simulation of our $k$-round asynchronous FL}
\label{subsec:kroundFL_simu}

In order to understand the behavior of the FL systems. We conduct the following experiments. 


\begin{table}[ht]
\caption{Federated Learning with different number of samples.}
\label{tbl_samples}
\vskip 0.1in
\begin{center}
\begin{small}
% \begin{sc}
\begin{tabular}{lcccr}
\toprule
Parameter & Value & Notes \\ [0.5ex]
\midrule
Learning rate $\eta$ & 0.001 &  fixed                       \\ 
% \hline
Data set & MNIST & $0$ and $1$ digit                \\
% \hline
Number of clients $n$ & 3 &                              \\
% \hline
Image size & 28x28   & grayscale                    \\
Train dataset records & 14867 &                          \\

% \hline
Number of samples $s$ & 10/50/100/500/1K/2K/\\ &2.5K/10K/15K &                  \\
% \hline
Number of round $r$ & 5 &                               \\
\bottomrule
\end{tabular}
% \end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

\begin{figure}[ht]
\includegraphics[width=\columnwidth]{tikz/01_fl_vary_sample_train_error.PNG}
\caption{FL with different number of samples.}
\label{fig:fl_sample}
\end{figure}

\vspace{0.2cm}
\noindent
\textbf{Varying the size of samples $s$ while fixing parameters $k,n$ and $\eta$:} The goal of this experiment is that $s$ can not be arbitrary large due to the restriction from the delay parameter $\tau$. To make the analysis simple, we consider $1$-round asynchronous FL (i.e., original FL). The detailed setup of this experiment for logistic regression problem is described in Table~\ref{tbl_samples}.

Figure~\ref{fig:fl_sample} reveals that when the number of samples $s=500$, we gain the highest accuracy. In addition, if we continue to increase the number of samples, the accuracy keeps nearly unchanged, i.e, large number of samples does not guarantee the improvement of accuracy.

\vspace{0.2cm}
\noindent
\textbf{Varying the number of clients $n$ while fixing parameters $k,s$ and $\eta$:} The goal of this experiment is that $n$ can not be arbitrary large due to the restriction from the delay parameter $\tau$. To make the analysis simple, we consider $1$-round asynchronous FL (i.e., original FL). \textcolor{red}{We choose the small stepsize for the simulation due to the fact that we need the large number of samples and clients to show that large number of clients can affect the train accuracy.} The detail parameters of this experiment are illustrated in Table~\ref{tbl_clients}.

\begin{table}[ht]
\caption{Federated Learning with different number of clients.}
\label{tbl_clients}
\vskip 0.1in
\begin{center}
\begin{small}
% \begin{sc}
\begin{tabular}{lcccr}
\toprule
Parameter & Value & Notes \\ [0.5ex]
\midrule
Learning rate $\eta$ & 0.00025 &  fixed                       \\ 
% \hline
Data set & MNIST & $0$ and $1$ digit                \\
% \hline
% \hline
Image size & 28x28   & grayscale                    \\
Data set records & 14867 &                          \\
% \hline
Number of clients $n$ & 5/10/20/30/40/50 &                  \\
Number of samples $s$ & 5000 &                  \\
% \hline
$k$-round & 5 &                               \\
\bottomrule
\end{tabular}
% \end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

\begin{figure}[ht]
\includegraphics[width=\columnwidth]{tikz/01_fl_vary_client.PNG}
\caption{FL with different number of clients.}
\label{fig:fl_client}
\end{figure}

Figure~\ref{fig:fl_client} shows that when number of client $n=30$, the training process gain the lowest train error, i.e, the largest accuracy while if $n$ continue to increase, the accuracy will dramatically decreases.

\vspace{0.2cm}
\noindent
\textbf{Varying the round parameter $k$ while fixing parameters $n,s$ and $\eta$:} The goal of this experiment is to verify the convergence rate of the system when $k$ increases. Table~\ref{tbl_k_round} defines the detail parameters of the experiment.


\begin{table}[ht]
\caption{Federated Learning with different number of $k$-round.}
\label{tbl_k_round}
\vskip 0.1in
\begin{center}
\begin{small}
% \begin{sc}
\begin{tabular}{lcccr}
\toprule
Parameter & Value & Notes \\ [0.5ex]
\midrule
Learning rate $\eta$ & 0.0001 &  fixed                         \\ 
% \hline
Data set & MNIST & $0$ and $1$ digit                    \\
% \hline
% \hline
Image size & 28x28   & grayscale                        \\
Data set records & 14867 &                              \\
% \hline
Number of clients $n$ & 3 &                                  \\
Number of samples $s$ & 1000 &                              \\
% \hline
Number of rounds & 5 &                                   \\
$k$-round & 1/2/3/4/5/6 & asyn-round of client                   \\
\bottomrule
\end{tabular}
% \end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

\begin{figure}[ht]
\includegraphics[width=\columnwidth]{tikz/01_fl_vary_k_round.PNG}
\caption{FL with different number of $k$-round.}
\label{fig:fl_k_round}
\end{figure}

As can be seen from Figure~\ref{fig:fl_k_round}, when we change the $k$-round value from 1 to 2 and 3, the train error goes down dramatically. It means that asynchronous FL helps the model converge faster than the traditional FL. However, when we continue to increase the value $k$, the train error almost remains unchanged.


\textcolor{red}{\textbf{Important Note}:} From the implementation, we have the following observation: assume that there exists a good $k$-asynchronous FL, i.e., the clients always get a new model $w$ from the server before finishing all $k$ rounds of computation. Then for any $k'(>k)$-round asynchronous FL, it should include that good $k$-round asynchronous one. This fact leads to the important following result: the clients always get the new model $w$ before finishing all $k$ rounds rather than $k'$ rounds. In other words, $k'$ can be arbitrary large or the clients seem never be in \textit{waiting mode} as described in Figure~\ref{fig:framework_waiting}. Therefore, the designer only needs to find the optimal numbers $s$ and $n$ and can ignore the parameter $k$ by setting it  large. This allows the clients and server to work in a fully asynchronous mode. 


\subsection{Real applications of Federated learning}

\textbf{Text prediction on Android phone}: We can create an Android phone for chatting purpose. Based on the text content from client, we can used it for training a text prediction model. We can take reference from Google Keyboard application \cite{GoogleAIBlog,hard2018federated}.

\textbf{Diseases Detection based on daily activities}: Based on mobile phone, we can collect behavioral data from client, for example, sleep time, exercise habit, daily activities. Certain activities in daily life can reflect early signals of some diseases, so we can create a mode for detecting common diseases. For example, without enough sleep, people can suffer from seizure or mental disorders \cite{chen2019fedhealth}.

\textbf{Music recommendation engine:} which recommends music on an app for users. Specifically, we can predict emoji from text typed on a mobile keyboard and then recommends appropriate music for users \cite{ramaswamy2019federated}.

\textbf{Fraud detection model:} multiple banks could train a common powerful fraud detection model without sharing their sensitive customer data with each other through Federated Learning.


\textcolor{red}{https://hackernoon.com/a-beginners-guide-to-federated-learning-b29e29ba65cf}


\textbf{Technologies and Frameworks for Federated Learning
:} Some of the popular and recent Federated Learning frameworks include TensorFlow Federated, an open source framework by Google for experimenting with machine learning and other computations on decentralized data. PySyft is a open source library that is built on top of PyTorch for encrypted, privacy preserving deep learning. Federated AI Technology Enabler (FATE) is an open-source project initiated by Webank’s AI group to provide a secure computing framework to support the Federated AI ecosystem.

Several new startups such as S20.ai, Owkin, and Snips have emerged in this space creating new tools and enterprise solutions around Federated Learning and other secure computation techniques across different verticals

\textbf{Federated Learning is still in its early stages and faces numerous challenges with its design and deployment.
}
For instance, its feasibility is highly constrained by the capabilities of the edge devices to perform local training and inferencing. While this may not remain a major barrier to entry as most smartphones and IoT devices newly launched are equipped with GPUs or sufficient computing hardware to run powerful AI models. Today it’s still impossible to train a network without compromising device performance and user experience or compressing a model and resorting to a lower accuracy.

Local training of supervised models requires labeled data which isn’t available or difficult to produce in most cases. A good way to tackle this challenge is by defining the Federated Learning problem and designing data pipeline such that labels are captured in an implicit way, for example, user’s interactions, feedback on model responses based on certain actions taken or events triggered, etc.

In real world cases, model convergence time is higher in the Federated setup as compared to the traditional central training approach. There could be reliability issues where not all devices participate in the Federated Learning process due to connectivity issues, different app usage patterns and model training times, irregular or missed updates, etc. Federated Learning should be considered only when the size of the data and cost of aggregating from distributed sources is very high. inconsistent model versions across the clients does not affect the experience too much for a significant time window and the central model can converge with minimal client participation.

Finally, the mindset of centrally aggregating data and creating silos by large companies for competitive advantage would be a major challenge to drive the adoption of Federated Learning. Effective data protection policies and appropriate incentives and business models around decentralizing data can tackle these issues and develop the Federated AI ecosystem















